Adversarial Robustness for Code

Machine learning and deep learning in particular has been recently used to successfully address many tasks in the domain of code such as finding and fixing bugs, code completion, decompilation, type inference and many others. However, the issue of adversarial robustness of models for code has gone largely unnoticed. In this work, we explore this issue by: (i) instantiating adversarial attacks for code (a domain with discrete and highly structured inputs), (ii) showing that, similar to other domains, neural models for code are vulnerable to adversarial attacks, and (iii) combining existing and novel techniques to improve robustness while preserving high accuracy.

==> figures/motivation.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}

\node (base) at (0,0) { 
\begin{lstlisting}[language=JavaScript, mathescape]
(hex$^\scode{str}$, radix$^\scode{num}$) => {
  v$^\scode{num}$ = parseInt$^\scode{num}$(
     hex.substring$^\scode{str}$(1), 
     radix
   );
  red = v >> 16$^\scode{num}$;
  ...
}
\end{lstlisting}
};


%\node[below=of base, yshift=1.0cm, font=\footnotesize] { $\E_{(x, y) \sim \dataset} [ \ell_{\scode{CrossEntropy}}(f(x), y) ]$};

\node[right= of base, xshift=-1.0cm] (adv) { 
\begin{lstlisting}[language=JavaScript, mathescape]
(hex$^\scode{str}$, radix$^\scode{num}$) => {
  v$^\scode{num}$ = parseInt$^\scode{num}$(
     hex.substring$^\scode{str}$(1), 
     radix
   );
  red = v >> 16$^\scode{num}$;
  ...
}
\end{lstlisting}
};


%\node[below=of base, yshift=1.0cm, font=\footnotesize] { $\E_{(x, y) \sim \dataset} [ \ell_{\scode{CrossEntropy}}(f(x), y) ]$};

\end{tikzpicture}
\caption{Caption.}
\end{figure}

==> tables/ablation.tex <==
\begin{table}[t]
\centering
\tra{1.1}

\caption{Robustness breakdown of models trained using a subset of the components proposed in our work.}
\tablabel{ablation}

\scalebox{0.88}{
\begin{tabular}{l c c c c c c} 
\toprule
 & & \multicolumn{3}{c}{Robustness}\\
\cmidrule(r){3-5}
$\quad$Dataset & Size & $\forall$ Correct & $\exists$ Incorrect & Abstain \\ 
\midrule
\footnotesize \lstma{} & \multicolumn{4}{l}{\footnotesize $t_\scode{acc}=1.00$ \textbf{Abstain}} \\
$\quad\dataset_{\scode{correct}}$ & $\;\;8.51\%$ & $0.13\%$ & $0.02\%$ & $99.85\%$ \\
$\quad\dataset_{\scode{abstain}}$ & $91.48\%$ & $-$ & $0.07\%$ & $99.93\%$ \\
\footnotesize \lstma{} & \multicolumn{4}{l}{\footnotesize $t_\scode{acc}=1.00$ \textbf{Abstain + Adversarial}} \\
$\quad\dataset_{\scode{correct}}$ & $\;\;8.67\%$ & $0.09\%$ & $0.03\%$ & $99.88\%$ \\
$\quad\dataset_{\scode{abstain}}$ & $91.32\%$ & $-$ & $0.23\%$ & $99.77\%$ \\

\footnotesize \gnn{} &\multicolumn{4}{l}{\footnotesize $t_\scode{acc}=1.00$ \textbf{Abstain}} \\
$\quad\dataset_{\scode{correct}}$ & $\;\;2.51\%$ & $14.44\%$ & $0.00\%$ & $85.56\%$ \\
$\quad\dataset_{\scode{abstain}}$ & $97.48\%$ & $-$ & $0.09\%$ & $99.91\%$ \\
\footnotesize \gnn{} &\multicolumn{4}{l}{\footnotesize $t_\scode{acc}=1.00$ \textbf{Abstain + Adversarial}} \\
$\quad\dataset_{\scode{correct}}$ & $\;\;2.03\%$ & $28.94\%$ & $0.00\%$ & $71.06\%$ \\
$\quad\dataset_{\scode{abstain}}$ & $97.96\%$ & $-$ & $0.25\%$ & $99.75\%$ \\

\bottomrule
\end{tabular}  
}


\end{table}


==> tables/baselines.tex <==
\begin{table*}[t]
\centering
\tra{1.2}
\caption{TODO}
\label{refinement_loop}
\begin{tabular}{r c c c c c c} 
  \toprule

& \multicolumn{3}{c}{Non-Adversarial Accuracy} & \multicolumn{3}{c}{Adversarial Accuracy} \\
\cmidrule(r){2-4} \cmidrule(r){5-7} 
Model & Correct & Incorrect & Reject & Correct & Reject & Total  \\ 
  \midrule
\multicolumn{4}{l}{\footnotesize \textbf{Standard Training}} \\
Sequence (LSTM) 	& $87.23\%$ & $12.77\%$ & $-$ & $2.87\%$ & $-$ & $2.51\%$\\ %Train Accuracy: 96.4
Graph (UTransfromer) 	& $88.10\%$ & $11.90\%$ & $-$ & $60.49\%$ & $-$ & $53.29\%$\\ %Train Accuracy: 97.32
\multicolumn{4}{l}{\footnotesize \textbf{Adversarial Training}} \\				
Sequence (LSTM) 	&  $87.84\%$ & $12.16\%$ & $-$ & $4.41\%$ & $-$ & $3.87\%$\\
Graph (UTransfromer) 	& $88.44\%$ & $11.56\%$ & $-$ & $59.58\%$ & $-$ & $52.70\%$\\
\multicolumn{4}{l}{\footnotesize \textbf{Standard Training + Reject ($o=1$)}} \\				
Sequence (LSTM) 	&   \\
Graph (UTransfromer) 	& $99.99\%$ & $0.01\%$ & $88.47\%$ \\
\multicolumn{4}{l}{\footnotesize \textbf{Adversarial Training + Reject ($o=1$)}} \\				
Sequence (LSTM) 	&  \\
Graph (UTransfromer) 	& \\
\multicolumn{4}{l}{\footnotesize \textbf{Standard Training + Reject ($o=1 + \epsilon$)}} \\				
Sequence (LSTM) 	&  \\
Graph (UTransfromer) 	& \\
\multicolumn{4}{l}{\footnotesize \textbf{Adversarial Training + Reject ($o=1 + \epsilon$)}} \\				
Sequence (LSTM) 	&  \\
Graph (UTransfromer) 	& \\
\multicolumn{4}{l}{\footnotesize \textbf{Standard Training + Reject ($o=1$) + Refinement (1 iteration)}} \\				
Sequence (LSTM) 	&  \\
Graph (UTransfromer) 	& \\
\multicolumn{4}{l}{\footnotesize \textbf{Adversarial Training + Reject ($o=1$) + Refinement (1 iteration)}} \\				
Sequence (LSTM) 	&  \\
Graph (UTransfromer) 	& \\

  \bottomrule
  \end{tabular}  

\end{table*}


